Exploring the Nexus Between Retrievability and Query Generation Strategies

Quantifying bias in retrieval functions through document retrievability scores is vital for assessing recall-oriented retrieval systems. However, many studies investigating retrieval model bias lack validation of their query generation methods as accurate representations of retrievability for real users and their queries. This limitation results from the absence of established criteria for query generation in retrievability assessments. Typically, researchers resort to using frequent collocations from document corpora when no query log is available. In this study, we address the issue of reproducibility and seek to validate query generation methods by comparing retrievability scores generated from artificially generated queries to those derived from query logs. Our findings demonstrate a minimal or negligible correlation between retrievability scores from artificial queries and those from query logs. This suggests that artificially generated queries may not accurately reflect retrievability scores as derived from query logs. We further explore alternative query generation techniques, uncovering a variation that exhibits the highest correlation. This alternative approach holds promise for improving reproducibility when query logs are unavailable.

==> correlation-table.tex <==
\begin{table*}[]
    \centering
    \caption{Correlation between retrievability scores when 
      computed using the real query set (AOL) and 
      % when they are computed 
      the four simulated query sets (discussed in
      Section~\ref{subsec:simu-queries}).
      Upper triangle contains Pearson's $r$ while lower
      triangle reports Kendall's rank correlation $\tau$.
      All differences statistically significant with $p
      < 0.05$.
      Highest and lowest correlations for each dataset highlighted with superscript $^\dagger$ and $^*$.
    }
    \label{tab:correl}
    \resizebox{1\columnwidth}{!}
    {
\begin{tabular}{||c||ccccc||ccccc||ccccc||}
  \hline
  & \multicolumn{5}{c||}{\textbf{Robust04}}   & \multicolumn{5}{c||}{\textbf{WT10g}}   & \multicolumn{5}{c||}{\textbf{Wikipedia}} \\ \hline % \cmidrule{2-16} % \cmidrule{7-11} \cmidrule{12-16}
  & \multicolumn{1}{c}{\textbf{$\mathsf{SQ_{1}}$}} & \multicolumn{1}{c}{\textbf{$\mathsf{SQ_{2}}$}} & \multicolumn{1}{c}{\textbf{$\mathsf{SQ_{3}}$}} & \multicolumn{1}{c}{\textbf{$\mathsf{RSQ}$}} & \multicolumn{1}{c||}{\textbf{$\mathsf{AOL}$}} & \multicolumn{1}{c}{\textbf{$\mathsf{SQ_{1}}$}} & \multicolumn{1}{c}{\textbf{$\mathsf{SQ_{2}}$}} & \multicolumn{1}{c}{\textbf{$\mathsf{SQ_{3}}$}} & \multicolumn{1}{c}{\textbf{$\mathsf{RSQ}$}} & \multicolumn{1}{c||}{\textbf{$\mathsf{AOL}$}} & \multicolumn{1}{c}{\textbf{$\mathsf{SQ_{1}}$}} & \multicolumn{1}{c}{\textbf{$\mathsf{SQ_{2}}$}} & \multicolumn{1}{c}{\textbf{$\mathsf{SQ_{3}}$}} & \multicolumn{1}{c}{\textbf{$\mathsf{RSQ}$}} & \multicolumn{1}{c||}{\textbf{$\mathsf{AOL}$}} \\\hline
  
% \textbf{$\mathsf{SQ_{1}}$} & ~   & 0.0923                  & -0.0025                 & 0.7549                  & 0.1250                  & ~   & 0.1206                  & 0.2094                  & 0.3103                  & 0.1100                  & ~   & 0.1586                  & 0.2613                  & 0.4768                  & 0.2379                  \\
% \textbf{$\mathsf{SQ_{2}}$} & 0.1758                  & ~   & -0.0004                 & 0.1461                  & 0.0033                  & 0.3575                  & ~   & 0.5503                  & 0.1931                  & 0.0900                  & 0.3508                  & ~   & 0.7019                  & 0.1599                  & 0.0598                  \\
% \textbf{$\mathsf{SQ_{3}}$} & 0.0108                  & -0.0040                 & ~   & 0.0030                  & 0.0165                  & 0.3223                  & 0.3047                  & ~   & 0.2535                  & 0.1795                  & 0.3897                  & 0.5116                  & ~   & 0.1048                  & 0.0308                  \\
% \textbf{$\mathsf{RSQ}$} & 0.5617                  & 0.3023                  & 0.0233                  & ~   & 0.2076                  & 0.5672                  & 0.5312                  & 0.3189                  & ~   & 0.3135                  & 0.5350                  & 0.4867                  & 0.3739                  & ~   & 0.3065                  \\
% \textbf{$\mathsf{AOL}$} & 0.1413                  & -0.0174                 & 0.0321                  & 0.1811                  & ~   & 0.3731                  & 0.2977                  & 0.3830                  & 0.4126                  & ~   & 0.3603                  & 0.3074                  & 0.2338                  & 0.4194                  & ~  \\
% \bottomrule

%%%%% + with middle lines in cells
% \textbf{$\mathsf{SQ_{1}}$}     & \multicolumn{1}{l|}{\cellcolor{gray!25}}       & \multicolumn{1}{r|}{~0.0923}  & \multicolumn{1}{r|}{-0.0025} & \multicolumn{1}{r|}{~0.7549} & ~0.1250                   & \multicolumn{1}{l|}{\cellcolor{gray!25}}       & \multicolumn{1}{r|}{~0.1206} & \multicolumn{1}{r|}{~0.2094} & \multicolumn{1}{r|}{~0.3103} & ~0.1100                   & \multicolumn{1}{l|}{\cellcolor{gray!25}}       & \multicolumn{1}{r|}{~0.1586} & \multicolumn{1}{r|}{~0.2613} & \multicolumn{1}{r|}{~\textbf{0.4768}} & ~0.2379                   \\ \hline
% \textbf{$\mathsf{SQ_{2}}$} & \multicolumn{1}{r|}{~0.1758} & \multicolumn{1}{l|}{\cellcolor{gray!25}}        & \multicolumn{1}{r|}{-0.0004} & \multicolumn{1}{r|}{~0.1461} & 0.0033                   & \multicolumn{1}{r|}{~0.3575} & \multicolumn{1}{l|}{\cellcolor{gray!25}}       & \multicolumn{1}{r|}{~0.5503} & \multicolumn{1}{r|}{~0.1931} & 0.0900                   & \multicolumn{1}{r|}{~0.3508} & \multicolumn{1}{l|}{\cellcolor{gray!25}}       & \multicolumn{1}{r|}{~0.7019} & \multicolumn{1}{r|}{~0.1599} & ~0.0598                   \\ \hline
% \textbf{$\mathsf{SQ_{3}}$} & \multicolumn{1}{r|}{~0.0108} & \multicolumn{1}{r|}{-0.0040} & \multicolumn{1}{l|}{\cellcolor{gray!25}}        & \multicolumn{1}{r|}{~0.0030} & 0.0165                   & \multicolumn{1}{r|}{~0.3223} & \multicolumn{1}{r|}{~0.3047} & \multicolumn{1}{l|}{\cellcolor{gray!25}}       & \multicolumn{1}{r|}{~0.2535} & 0.1795                   & \multicolumn{1}{r|}{~0.3897} & \multicolumn{1}{r|}{~0.5116} & \multicolumn{1}{l|}{\cellcolor{gray!25}}       & \multicolumn{1}{r|}{~0.1048} & 0.0308                   \\ \hline
% \textbf{$\mathsf{RSQ}$} & \multicolumn{1}{r|}{~0.5617} & \multicolumn{1}{r|}{~0.3023}  & \multicolumn{1}{r|}{~0.0233}  & \multicolumn{1}{l|}{\cellcolor{gray!25}}       & 0.2076                   & \multicolumn{1}{r|}{~0.5672} & \multicolumn{1}{r|}{~0.5312} & \multicolumn{1}{r|}{~0.3189} & \multicolumn{1}{l|}{\cellcolor{gray!25}}       & 0.3135                   & \multicolumn{1}{r|}{~0.5350} & \multicolumn{1}{r|}{~0.4867} & \multicolumn{1}{r|}{~0.3739} & \multicolumn{1}{l|}{\cellcolor{gray!25}}       & 0.3065                   \\ \hline
% \textbf{$\mathsf{AOL}$} & \multicolumn{1}{r|}{~0.1413} & \multicolumn{1}{r|}{-0.0174} & \multicolumn{1}{r|}{~0.0321}  & \multicolumn{1}{r|}{~0.1811} & \multicolumn{1}{l||}{\cellcolor{gray!25}}    & \multicolumn{1}{r|}{~0.3731} & \multicolumn{1}{r|}{~0.2977} & \multicolumn{1}{r|}{~0.3830} & \multicolumn{1}{r|}{~0.4126} & \multicolumn{1}{l||}{\cellcolor{gray!25}}    & \multicolumn{1}{r|}{~0.3603} & \multicolumn{1}{r|}{~0.3074} & \multicolumn{1}{r|}{~0.2338} & \multicolumn{1}{r|}{~0.4194} & \multicolumn{1}{l||}{\cellcolor{gray!20}}    \\ \hline
% %%%%% - with middle lines in cells
% % \\ \hline
% % 

\textbf{$\mathsf{SQ_{1}}$}     & \multicolumn{1}{l}{\cellcolor{gray!25}}       & \multicolumn{1}{l}{~0.0923}  & \multicolumn{1}{l}{-0.0025} & \multicolumn{1}{l}{~{0.7549$^\dagger$}} & 0.1250~                   & \multicolumn{1}{l}{\cellcolor{gray!25}}       & \multicolumn{1}{l}{~0.1206} & \multicolumn{1}{l}{~0.2094} & \multicolumn{1}{l}{~0.3103} & ~0.1100                   & \multicolumn{1}{l}{\cellcolor{gray!25}}       & \multicolumn{1}{l}{~0.1586} & \multicolumn{1}{l}{~0.2613} & \multicolumn{1}{l}{~0.4768} & ~0.2379                   \\ \hline
\textbf{$\mathsf{SQ_{2}}$} & \multicolumn{1}{l}{~0.1758} & \multicolumn{1}{l}{\cellcolor{gray!25}}        & \multicolumn{1}{l}{-0.0004$^*$} & \multicolumn{1}{l}{~0.1461} & 0.0033                   & \multicolumn{1}{l}{~0.3575} & \multicolumn{1}{l}{\cellcolor{gray!25}}       & \multicolumn{1}{l}{~{0.5503}$^\dagger$} & \multicolumn{1}{l}{~0.1931} & 0.0900$^*$                   & \multicolumn{1}{l}{~0.3508} & \multicolumn{1}{l}{\cellcolor{gray!25}}       & \multicolumn{1}{l}{~{0.7019}$^\dagger$} & \multicolumn{1}{l}{~0.1599} & ~0.0598                   \\ \hline
\textbf{$\mathsf{SQ_{3}}$} & \multicolumn{1}{l}{~0.0108} & \multicolumn{1}{l}{-0.0040$^*$} & \multicolumn{1}{l}{\cellcolor{gray!25}}        & \multicolumn{1}{l}{~0.0030} & 0.0165                   & \multicolumn{1}{l}{~0.3223} & \multicolumn{1}{l}{~0.3047} & \multicolumn{1}{l}{\cellcolor{gray!25}}       & \multicolumn{1}{l}{~0.2535} & 0.1795                   & \multicolumn{1}{l}{~0.3897} & \multicolumn{1}{l}{~0.5116} & \multicolumn{1}{l}{\cellcolor{gray!25}}       & \multicolumn{1}{l}{~0.1048} & \multicolumn{1}{l||}{0.0308$^*$}                   \\ \hline
\textbf{$\mathsf{RSQ}$} & \multicolumn{1}{l}{~{0.5617}$^\dagger$} & \multicolumn{1}{l}{~0.3023}  & \multicolumn{1}{l}{~0.0233}  & \multicolumn{1}{l}{\cellcolor{gray!25}}       & 0.2076                   & \multicolumn{1}{l}{~{0.5672}$^\dagger$} & \multicolumn{1}{l}{~0.5312} & \multicolumn{1}{l}{~0.3189} & \multicolumn{1}{l}{\cellcolor{gray!25}}       & 0.3135                   & \multicolumn{1}{l}{~{0.5350}$^\dagger$} & \multicolumn{1}{l}{~0.4867} & \multicolumn{1}{l}{~0.3739} & \multicolumn{1}{l}{\cellcolor{gray!25}}       & 0.3065                   \\ \hline
\textbf{$\mathsf{AOL}$} & \multicolumn{1}{l}{~0.1413} & \multicolumn{1}{l}{-0.0174} & \multicolumn{1}{l}{~0.0321}  & \multicolumn{1}{l}{~0.1811} & \multicolumn{1}{l||}{\cellcolor{gray!25}}    & \multicolumn{1}{l}{~0.3731} & \multicolumn{1}{l}{~0.2977$^*$} & \multicolumn{1}{l}{~0.3830} & \multicolumn{1}{l}{~0.4126} & \multicolumn{1}{l||}{\cellcolor{gray!25}}    & \multicolumn{1}{l}{~0.3603} & \multicolumn{1}{l}{~0.3074} & \multicolumn{1}{l}{~0.2338$^*$} & \multicolumn{1}{l}{~0.4194} & \multicolumn{1}{l||}{\cellcolor{gray!20}}    \\ \hline

\end{tabular}
}
\vspace{-3mm}
\end{table*}




% \begin{table}[]
% \begin{tabular}{|l|rrrrr|rrrrr|rrrrr|}
% \hline
%     & \multicolumn{5}{c|}{Robust04}                                                                                                                      & \multicolumn{5}{c|}{WT10g}                                                                                                                       & \multicolumn{5}{c|}{Wikipedia}                                                                                                                   \\ \hline
%     & \multicolumn{1}{l|}{SQ1}    & \multicolumn{1}{l|}{SQ2}     & \multicolumn{1}{l|}{SQ3}     & \multicolumn{1}{l|}{RSQ}    & \multicolumn{1}{l|}{AOL} & \multicolumn{1}{l|}{SQ1}    & \multicolumn{1}{l|}{SQ2}    & \multicolumn{1}{l|}{SQ3}    & \multicolumn{1}{l|}{RSQ}    & \multicolumn{1}{l|}{AOL} & \multicolumn{1}{l|}{SQ1}    & \multicolumn{1}{l|}{SQ2}    & \multicolumn{1}{l|}{SQ3}    & \multicolumn{1}{l|}{RSQ}    & \multicolumn{1}{l|}{AOL} \\ \hline
%     % 
%     & \multicolumn{1}{l|}{}       & \multicolumn{1}{r|}{0.0923}  & \multicolumn{1}{r|}{-0.0025} & \multicolumn{1}{r|}{0.7549} & 0.1250                   & \multicolumn{1}{l|}{}       & \multicolumn{1}{r|}{0.1206} & \multicolumn{1}{r|}{0.2094} & \multicolumn{1}{r|}{0.3103} & 0.1100                   & \multicolumn{1}{l|}{}       & \multicolumn{1}{r|}{0.1586} & \multicolumn{1}{r|}{0.2613} & \multicolumn{1}{r|}{0.4768} & 0.2379                   \\ \hline
% SQ2 & \multicolumn{1}{r|}{0.1758} & \multicolumn{1}{l|}{}        & \multicolumn{1}{r|}{-0.0004} & \multicolumn{1}{r|}{0.1461} & 0.0033                   & \multicolumn{1}{r|}{0.3575} & \multicolumn{1}{l|}{}       & \multicolumn{1}{r|}{0.5503} & \multicolumn{1}{r|}{0.1931} & 0.0900                   & \multicolumn{1}{r|}{0.3508} & \multicolumn{1}{l|}{}       & \multicolumn{1}{r|}{0.7019} & \multicolumn{1}{r|}{0.1599} & 0.0598                   \\ \hline
% SQ3 & \multicolumn{1}{r|}{0.0108} & \multicolumn{1}{r|}{-0.0040} & \multicolumn{1}{l|}{}        & \multicolumn{1}{r|}{0.0030} & 0.0165                   & \multicolumn{1}{r|}{0.3223} & \multicolumn{1}{r|}{0.3047} & \multicolumn{1}{l|}{}       & \multicolumn{1}{r|}{0.2535} & 0.1795                   & \multicolumn{1}{r|}{0.3897} & \multicolumn{1}{r|}{0.5116} & \multicolumn{1}{l|}{}       & \multicolumn{1}{r|}{0.1048} & 0.0308                   \\ \hline
% RSQ & \multicolumn{1}{r|}{0.5617} & \multicolumn{1}{r|}{0.3023}  & \multicolumn{1}{r|}{0.0233}  & \multicolumn{1}{l|}{}       & 0.2076                   & \multicolumn{1}{r|}{0.5672} & \multicolumn{1}{r|}{0.5312} & \multicolumn{1}{r|}{0.3189} & \multicolumn{1}{l|}{}       & 0.3135                   & \multicolumn{1}{r|}{0.5350} & \multicolumn{1}{r|}{0.4867} & \multicolumn{1}{r|}{0.3739} & \multicolumn{1}{l|}{}       & 0.3065                   \\ \hline
% AOL & \multicolumn{1}{r|}{0.1413} & \multicolumn{1}{r|}{-0.0174} & \multicolumn{1}{r|}{0.0321}  & \multicolumn{1}{r|}{0.1811} & \multicolumn{1}{l|}{}    & \multicolumn{1}{r|}{0.3731} & \multicolumn{1}{r|}{0.2977} & \multicolumn{1}{r|}{0.3830} & \multicolumn{1}{r|}{0.4126} & \multicolumn{1}{l|}{}    & \multicolumn{1}{r|}{0.3603} & \multicolumn{1}{r|}{0.3074} & \multicolumn{1}{r|}{0.2338} & \multicolumn{1}{r|}{0.4194} & \multicolumn{1}{l|}{}    \\ \hline
% \end{tabular}
% \end{table}

% %%% Local Variables:
% %%% mode: latex
% %%% TeX-master: "samplepaper"
% %%% End:


==> pos-based-query-generation.tex <==
\subsection{A POS-based query generation technique}\label{subsec:rule_simulation}

The contrasting nature of simulated queries, when compared to real queries, is briefly reported in~\cite{traub2016querylog}. According to their observation, the real queries contain a significantly higher fraction of named entities compared to the simulated query set.
Inspired by this observation, we propose a part of speech based query generation technique in this section. 



The identification of collocations within a text corpus can be achieved through a straightforward counting approach, whereby the frequency of co-occurring word pairs is examined. This technique provides evidence of words that possess a distinct function, one that extends beyond a mere combination of their individual meanings. However, the process of selecting the most frequent bigrams alone often yields uninteresting results. Upon closer inspection, it becomes apparent that a substantial portion of these bigrams consists of function words, offering limited insights. To enhance the quality of identified collocations, a simple yet effective heuristic was proposed by Justeson and Katz~\cite{justeson1991co}. This heuristic involves subjecting candidate phrases to a part-of-speech filter, which selectively retains patterns likely to represent genuine ``phrases" rather than random word combinations. Justeson and Katz specifically recommend certain tag patterns for both bigrams and trigrams, enhancing the meaningfulness of the resulting collocation identification process.

Therefore, to enhance the process of identifying collocations, we propose to integrate Justeson and Katz's part-of-speech filtering method into the query generation approach. By incorporating this technique, we aim to selectively extract the most "query-like" N-grams, thereby improving the relevance and effectiveness of the generated queries. Our improved method introduces the following additional steps to the existing procedure:
\begin{enumerate}
    \item Perform Part-of-Speech (POS) tagging on the collection documents: Initially, we employ POS tagging on all the documents within the collection. This step assigns appropriate grammatical tags to each word, facilitating the subsequent identification of N-grams.
    \item Extract N-grams from the POS-tagged documents: N-grams, where N represents the desired length of the word sequences, are extracted from the POS-tagged documents. In our case, we consider N to range from 1 to 4, enabling the identification of unigrams, bigrams, trigrams, and quadgrams.
    \item Select N-grams with ``query-like" POS tag patterns: From the pool of extracted N-grams, we apply Justeson and Katz's recommended POS tag patterns to filter and retain N-grams that exhibit patterns resembling queries. The specific POS tag patterns for each N-gram type are provided in Table \ref{tab:pos-tag}. Tag patterns for Quadgrams are proposed by us heuristically from our observations.
\end{enumerate}

Subsequently, the resulting list of N-grams is sorted in descending order based on their occurrence frequencies. To ensure a manageable and relevant set of queries, we truncate the list at specific thresholds. These thresholds are determined by drawing inspiration from the frequency distribution of queries found in the AOL query set~\cite{aol-log}. We aim to maintain a proportional ratio between the selected N-grams and the query frequencies observed in the AOL based real query set, thus preserving a close alignment with real-world query usage patterns.

\begin{table}[t]
\centering
\caption{POS Tag rules for N-grams query generation}
\label{tab:pos-tag}
\resizebox{0.99\columnwidth}{!}{
\renewcommand{\arraystretch}{2.0}
\begin{tabular}{|l|l|l|l|}
\hline
\textbf{Unigram}                & \textbf{Bigram}  & \textbf{Trigram}       & \textbf{Quadgram}     \\ \hline
NOUN                                      & ADJ NOUN                                & ADJ ADJ NOUN                                  & NOUN VERB ADP NOUN                                  \\ \hline
                                           & NOUN NOUN                              & ADJ NOUN NOUN                                 & ADJ NOUN ADJ NOUN                                   \\ \hline
                                           & & NOUN ADJ NOUN                          & NOUN ADP ADJ NOUN \\ \hline
                                           & & NOUN NOUN NOUN                         & NOUN NOUN ADP NOUN                                 \\ \hline
                                           & & NOUN ADP NOUN                          & NOUN VERB NOUN NOUN \\ \hline
                                           &                                       &                                               & ADV ADJ NOUN NOUN                                     \\ \hline
                                           &                                       &                                               & ADJ NOUN VERB NOUN                                  \\ \hline
                                           &                                       &                                               & NOUN ADJ NOUN NOUN                                     \\ \hline
\end{tabular}
}
\end{table}


==> ret.tex <==
Once a suitable query set has been generated, a retrieval model with a suitable parameter is chosen for performing the retrieval together with selecting a rank cutoff within which a document ranking will be considered. 
Then the retrievals with the set of queries are performed which itself is a time-consuming process.
The retrievability scores of the documents are then computed based on their position in the rank list after each retrieval.
Once the retrievability of the set of documents is computed retrieved after the retrieval with all the queries, 

With the results of each query recorded up to rank cutoff c, the computation of document retrievability r(d) can begin based on the selection of the utility function, either cumulative or gravity-based. 
Studies reported that these two measures are highly correlated ~\cite{wilkie2013relating, bashir2010improving} and hence later studies only report their analysis of retrievability computed based on either of the utility functions with the cumulative-based function being the popular choice.

With the utility function chosen and configured the r(d) for every document in the collection is computed. The result is a list of each document in the collection and its corresponding retrievability score(s). This list can be used to identify documents that are overly/underly retrievable [Bashir and Rauber, 2009b, Bashir and Rauber, 2009a] and can be used for improving pseudo relevance feedback [Bashir and Rauber, 2010a, Bashir and Rauber, 2010b].

The final step is the summarisation of the retrievability scores in a collection to quantify the bias present in the collection.
The most popular way to do so is by employing Gini coefficient, a measure popularly applied in the field of economics and social science to quantify the inequality persisting in a population. Other inequality metrics are also explored in~\cite{wilkie2015retrievability} where the authors argue that the inequality metrics generally agreed on which system and settings minimised the retrievability bias although there were differences between settings in terms of magnitude.




However, a common next step is to attempt to summarise the level of retrievability bias present
in a system. The common way to do this, as described earlier, is through the use of the Lorenz
Curve [Gastwirth, 1962] to estimate the Gini Coefficient. However, the Gini Coefficient is one
of a suite of inequality metrics and as such Wilkie and Azzopardi explored a set of inequality
metrics to determine their impact in the process of calculating retrievability bias [Wilkie and
Azzopardi, 2015]. Prior to this study, only the Gini Coefficient had been used to calculate
the overall retrievability bias and so the aim of this work was to examine whether or not
Gini was a suitable metric and if other metrics provided complimentary outlooks on bias.
Wilkie and Azzopardi performed a retrievability analysis on the Aquaint and .Gov collections
using 3 parameterised retrieval models: BM25, PL2 and LMD. Once they had retrievability
scores for a model and its settings, they calculated system retrievability bias using one of
6 inequality metrics and compared the estimation presented by each. The authors posited
that the inequality metrics generally agreed on which system and settings minimised the
retrievability bias although there were differences between settings in terms of magnitude. In
particular, they found that Palma Index [Palma, 2011] and the 20:20 Ratio both emphasised
the difference in magnitude between settings but they do still agree with the Gini Coefficient
and other measures. These findings were replicated across the combinations of retrieval
models and document collections. Due to this, the authors believed that continuing use of the
Gini Coefficient to summarise retrievability bias was not only acceptable but recommended
as the other metrics explored offered no argument otherwise. This work helped validate
Azzopardi and Vinay’s choice of inequality metric [Azzopardi and Vinay, 2008b] and means
that prior work is not challenged by its choice of inequality metric.




the system being assessed must be configured.
This stage entails choosing the model as well as setting any hyper-parameters associated with
the model in a way that fits the needs of your analysis. Often, researchers will perform a
retrievability analysis on a parameter sweep of the length normalisation parameter of a given
retrieval algorithm [Azzopardi and Vinay, 2008b, Wilkie and Azzopardi, 2013a, Wilkie and
Azzopardi, 2013b]. This step is simplistic and serves only to dictate what instantiation of
a system is being assessed. Following the set up of the system, the query set is issued to
the system one after the other. This stage is generally very time consuming given the large
volume of queries being issued. The results of each query are recorded and most systems will
allow a rank cutoff to be set which dictates how deep the ranking is. All documents ranked
after the cutoff are ignored. It is important that the cutoff set here is high enough that one can
compute the retrievability at the chosen cutoff. The outcome of this step is a ranked list of
results for every query in the query set used.
